OSOUM Framework for Trading Data Research

In the last decades, data have become a cornerstone component in many business decisions, and copious resources are being poured into production and acquisition of the high-quality data. This emerging market possesses unique features, and thus came under the spotlight for the stakeholders and researchers alike. In this work, we aspire to provide the community with a set of tools for making business decisions, as well as analysis of markets behaving according to certain rules. We supply, to the best of our knowledge, the first open source simulation platform, termed Open SOUrce Market Simulator (OSOUM) to analyze trading markets and specifically data markets. We also describe and implement a specific data market model, consisting of two types of agents: sellers who own various datasets available for acquisition, and buyers searching for relevant and beneficial datasets for purchase. The current simulation treats data as an infinite supply product. Yet, other market settings may be easily implemented using OSOUM. Although commercial frameworks, intended for handling data markets, already exist, we provide a free and extensive end-to-end research tool for simulating possible behavior for both buyers and sellers participating in (data) markets.

==> 05_eval.tex <==

\todo{bla bla bla}

\subsection{Empirical Settings}\label{sec:set}

\subsection{Simulation of a Data Market}

\subsection{Methodology}

\subsection{Evaluation Measures}

\subsection{Results}\label{sec:res}


